Practical Subarchitectures for Optimal Quantum Layout Synthesis

Quantum Layout Synthesis (QLS) maps a logical quantum circuit to a physical quantum platform. Optimal QLS minimizes circuit size and depth, which is essential to reduce the noise on current quantum platforms. Optimal QLS is an NP-hard problem, so in practice, one maps a quantum circuit to a subset of the complete quantum platform. However, to guarantee optimality, one still has to consider exponentially many subarchitectures. We introduce an effective method to enumerate relevant subarchitectures. This reduces the number of considered subarchitectures, as well as the number of expensive subgraph isomorphism checks, thus boosting Optimal QLS with subarchitectures. To do so, we assume a fixed number of ancilla qubits that can be used in the mapping. We guarantee optimality of the quantum layout, for the selected ancilla bound. We evaluate our technique on a number of benchmarks and compare it with state-of-the-art Optimal QLS tools with and without using subarchitectures.

==> figures/data/mqt40.tex <==
1.16326880455017						0.355016231536865
1.15663290023804						0.337291240692139
1.25657367706299						0.466248273849487
674.145435094833						470.660633802414
19.2895185947418						17.7890226840973
13.23570561409						114.212035417557
15.938545703888						9.85341143608093
3263.97587323189						136.605059623718
40.1112439632416						47.7563858032227
672.837249040604						371.032805204391
674.520728349685						472.362770318985
663.801820039749						370.0939245224
1.42974352836609						0.651477813720703
1.61698365211487						0.861088037490845
1.91372489929199						0.256737947463989
1.88813495635986						0.247056007385254
2.1068606376648						0.295931816101074
805.399454593659						391.750525712967
21.641535282135						1.83838629722595
50.1071307659149						10.5690014362335
73.5814554691315						27.7783393859863
4275.60899066925						656.272893667221
60.9031319618225						8.99557662010193
798.987704992294						385.750435352325
799.060263633729						389.5176923275
796.962942123413						389.978084802628
2.39656734466553						0.414814472198486
2.54901981353761						0.456897974014282
2100.92553257942						0.418598175048828
2101.43408989906						0.393469333648682
2131.20925879478						0.490389347076416
2288.26884698868						1.68185639381409
9977.11008000373						19.3170266151428
4225.84047865868						6.32768821716309
2125.7101688385						0.696501016616822
2118.12419223785						0.861352920532227


==> figures/data/mqt40_gates.tex <==
11						11
0						0
18						18
137						137
49						43
68						78
54						54
105						105
72						72
137						142
137						137
137						142
0						0
16						16
14						14
0						4
11						11
120						120
28						28
68						68
64						64
91						91
56						56
120						120
120						120
120						120
0						8
16						16
4						7
0						0
4						4
0						0
22						40
22						30
0						0
14						15


==> figures/data/mqt40_timeout.tex <==
100000						2268.34428620339
100000						32.5148582458496
100000						67.968540430069
100000						22.3536586761475
100000						33.2379059791565
100000						33.3415448665619
100000						30.5396165847779


==> figures/data/mqt41.tex <==
1.16326880455017						1.12766146659851
1.15663290023804						0.529427289962769
1.25657367706299						1.62713098526001
674.145435094833						1540.67477822304
19.2895185947418						88.7993383407593
13.23570561409						70.7236530780792
15.938545703888						83.9620089530945
40.1112439632416						101.35121011734
672.837249040604						1551.74525976181
674.520728349685						2299.00464081764
663.801820039749						1539.53593635559
1.42974352836609						1.01211094856262
1.61698365211487						3.32973146438599
1.91372489929199						1.66564393043518
1.88813495635986						1.07783770561218
2.1068606376648						2.44307136535645
805.399454593659						7660.64285349846
21.641535282135						85.1077909469605
50.1071307659149						233.402257680893
73.5814554691315						228.190859794617
60.9031319618225						966.161569833755
798.987704992294						7468.53134322166
799.060263633729						7426.67570447922
796.962942123413						7474.7105448246
2.39656734466553						2.43382954597473
2.54901981353761						4.08747220039368
2100.92553257942						1.81098771095276
2101.43408989906						0.520366191864014
2131.20925879478						2.3124144077301
2288.26884698868						12.9698083400727
9977.11008000373						371.309942245483
4225.84047865868						127.582269191742
2125.7101688385						1.076815366745
2118.12419223785						4.04402446746826


==> figures/data/mqt41_gates.tex <==
11						11
0						0
18						14
137						137
49						43
68						68
54						54
72						72
137						137
137						137
137						137
0						0
16						16
14						7
0						0
11						7
120						98
28						14
68						54
64						47
56						51
120						110
120						110
120						110
0						0
16						16
4						4
0						0
4						4
0						0
22						22
22						22
0						0
14						14


==> figures/data/mqt41_timeout.tex <==
3263.97587323189						100000
4275.60899066925						100000
100000						100000
100000						7993.43940377235
100000						6676.14416813851
100000						431.172288417816
100000						2483.06159520149
100000						2472.30107212067
100000						7987.74788355827


==> figures/data/qsynth_large.tex <==
5.2			0.18
0.17			0.02
0.02			0.01
1.02			0.19
3.54			4.08
1.32			0.1
136.88			16.7
0.15			0
0.02			0
5384.29			371.08
0.09			0.02
0.14			0.07
70.34			15.48
4830.15			32.98
331.02			10.39
128.17			7.9
0.39			0.14
167.99			39.89
6.97			3
807.57			52.91
12.61			4.15
1.96			1.27
0.12			0.92
0.17			1.2
0.2			5.72
0.2			1.79
0.2			60.77
0.19			54.07
6.47			0.29
0.46			0.01
0.05			0
13.18			1.61
55.2			16.78
0.13			6.82
2.89			0.02
95.21			148.62
0.31			0
0.05			0
8907.42			3917.26
0.18			0.06
0.24			0.79
121.93			50.71
1643.4			461.54
2386.42			338.43
513.64			58.92
0.67			0.14
6093.9			188.52
57.62			10.75
5555.75			276.83
35.03			12.56
7771.07			181.95
32.97			7.73
0.28			0.13
7.21			10.92
42.95			2058.48
3877.86			7795.29
571.11			0.89
1.6			0.02
5.5			0.01
45.16			1.65
977.7			17.12
0.3			0.8
6.78			0.05
1.28			0
0.13			0
9.43			0.09
17.55			0.74
696.55			8.3
6929.99			20.27
5.1			0.1
1493.69			11
600.55			9.08
256.83			6.78


==> figures/data/qsynth_large_timeout.tex <==
0.05			100000
0.07			100000
0.08			100000
0.08			100000
0.09			100000
0.08			100000
3.07			100000
0.45			100000
0.06			100000
100000			100000
100000			48.03
22.99			100000
100000			100000
100000			947.7
4684.05			100000
100000			100000
100000			100000
100000			100000
100000			60.17
100000			4497.62
100000			100000
100000			111.03
100000			91.56
100000			104.86
100000			207.3
100000			437.72


==> figures/data/qsynth_small.tex <==
0.01			0.01
0.55			0.55
2238.61			2218.58
2.71			1.09
0.03			0.02
0.04			0.01
1.85			2.15
18.27			26.66
0.01			0.03
0.06			0.06
38.28			812.87
0.01			0
0			0
1413.57			2226.37
0.1			0.11
0.56			1.49
4.1			25.06
149.83			483.65
233.38			1512.6
17.42			65.21
0.06			0.32
419.25			424.88
22.71			31.68
4485.07			1475.89
6.32			45.97
2972.75			695.11
2.84			8.68
0.01			0.01
0.01			0.01
0.01			0.01
0.01			0.02
0.01			0.02
0.02			0.02
0.52			0.19
0.04			0.01
0			0.01
0.4			1.35
14.9			27.6
0.01			0.03
0.25			0.09
25.54			99.66
0.01			0
0			0
0.01			0.04
0.37			0.6
2.19			36.58
16.51			501.7
14.41			101.72
6.26			13.02
0.04			0.1
43.71			154.8
1.34			31.13
48.79			268.66
1.52			36.22
41.68			233.24
0.64			6.9
0.01			0.17
0.02			0.23
0.02			0.26
0.03			0.95
0.02			0.4
0.02			0.45
0.01			0.14
0.01			0
0.01			0
0.01			0.01
0.01			3.14
0.02			0.83
0.01			0.01
1.4			11.31
0			0
0.01			0
12.38			25.75
1.08			886.71
0.01			0.03
0.01			0.08
0.02			1.99
9.66			15.12
3.54			3.88
2.99			6.19
0.01			0.02
6.11			14.59
0.39			0.88
19.75			45.61
0.37			0.76
18.12			24.38
0.03			0.34


==> figures/data/qsynth_small_timeout.tex <==
100000			100000
100000			100000
100000			100000
100000			100000
856.03			100000
100000			100000

